Finding the Needle in a Haystack: On the Automatic Identification of Accessibility User Reviews

In recent years, mobile accessibility has become an important trend with the goal of allowing all users the possibility of using any app without many limitations. User reviews include insights that are useful for app evolution. However, with the increase in the amount of received reviews, manually analyzing them is tedious and time-consuming, especially when searching for accessibility reviews. The goal of this paper is to support the automated identification of accessibility in user reviews, to help technology professionals in prioritizing their handling, and thus, creating more inclusive apps. Particularly, we design a model that takes as input accessibility user reviews, learns their keyword-based features, in order to make a binary decision, for a given review, on whether it is about accessibility or not. The model is evaluated using a total of 5,326 mobile app reviews. The findings show that (1) our model can accurately identify accessibility reviews, outperforming two baselines, namely keyword-based detector and a random classifier; (2) our model achieves an accuracy of 85% with relatively small training dataset; however, the accuracy improves as we increase the size of the training dataset.

==> Camera_Ready.tex <==
Please check Camera\_Ready.pdf file for details. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Start: Authors Information %%%%%%%%%%%%%%%%%%%%%%%%%%

Mohamed Wiem Mkaouer
Department of Software Engineering
Rochester Institute of Technology
Rochester, New York, United States
mwmvse@rit.edu


Yasmine N. El-Glaly
Department of Computer Science 
Western Washington University
Bellingham , Washington, United States
elglaly@wwu.edu


Murtaza Tamjeed 
Department of Software Engineering
Rochester Institute of Technology
Rochester, New York, United States
mt1256@rit.edu


Wajdi Aljedaani
Department of Computer Science and Engineering, University of North Texas
Denton, Texas, United States
wajdialjedaani@my.unt.edu


William Catzin
College of Engineering
University of California
Berkeley, California
williamcatzin@berkeley.edu


Eman Abdullah AlOmar 
Department of Software Engineering
Rochester Institute of Technology
Rochester, New York, United States
eman.alomar@mail.rit.edu

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End: Authors Information %%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Start: Summary of Changes (Required) %%%%%%%%%%%%%%
Please provide a brief summary of the changes you have made in preparation for the revised manuscript to address comments from the ACs. This summary will assist ACs in determining whether the terms of conditional acceptance have been satisfied.


In the revision, we have addressed the comments promised in the rebuttal as well as the point raised by the chairs:
(1) The changes promised in the rebuttal 
1.1: Clarify the cross-validation hold out testing set in sec 3.5
Section 3.5, Page 8, Line 827-833
1.2: Add details about the ML models in sec 3.4
Section 3.4, Page 6, Line 626-665
1.3: Add examples for false positives and false negatives in sec 4
Section 4, Page 8, Line 912-985 + Table 5
Section 3.5, Page 6-8, Line 694-830
1.4: Provide further analysis on the misspelled words in sec 4
Section 4, Page 8, Line 1244-1280 + Table 5
1.5: Provide more details on the features (e.g., keywords, context, semantics) used by the ML model in sec 4
Section 3.3, Page 6, Line 588-598
Section 4, page 8, Line 892-905 + Tables 3 & 4
1.6: Add a link to the public service and the dataset, in sec 1.
Section 1, Page 1, Line 213-220
1.7: Add details about the dataset and how it is realistic (information about the apps and reviews), in sec 3.1.
Section 3.1, Pages 4 & 5, Line 431-446 + Table 1 & Figure 2
1.8: Strengthen the discussion on the findings between ML and keyword-based approaches and adding examples of misspelled words to show how keyword-based fails while ML succeeds, in sec 4.2.
Section 4, Pages 11 - 13, Line 1244-1280 
1.9: Elaborate on the paper’s impact by explaining how future research can build on this paper in sec 5.
Section 5, Pages 12 & 13, Line 1370-1391 + Line 1445-1499
Section 7: Page 14, Line 1547-1558


(2) The usefulness of the method in practice was the primary reason for acceptance, but the case for usefulness will need to be improved in the paper. First, the paper should include more discussion about how developers could use the tool in practice (and perhaps even how this may compare to alternative approaches like manually reading the reviews or keywords alone). Second, the paper should add a discussion of the use case of people with disabilities filtering reviews when searching for apps to use. Users with disabilities may benefit from reading accessibility reviews before downloading and trying out an application. This use case convinced many PC members of the immediate utility of the tool.
Section 5, Pages 12 & 13, Line 1370-1391 + Line 1445-1499
Section 7: Page 14, Line 1547-1558

(3) The source code for the tool: 
We open source the code to make the tool immediately useful. The link can be found in: https://smilevo.github.io/access/index.html


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End: Summary of Changes (Required) %%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Start: General Information %%%%%%%%%%%%%%%%%%%%%%%%

Grant Agency: This material is based upon work supported by the National Science Foundation, USA, under Grant No. 1757680.

Presenting Author: 

Backup Presenting Author: 

Video Preview (Optional): Mohamed Wiem Mkaouer (ToDo)
You can submit an accompanying 30 second Video preview as a .mp4 file. The deadline for video previews is January 29th and should not exceed 20 MB. Note that the January 29th deadline is for the preview video only, do not delay the rest of your submission. See Technical Requirements and Guidelines for Videos at CHI for details.

Video Preview Captions (Required if the video preview contains spoken dialog): 
Subtitle file in .srt format. A manually created caption file is strongly recommended as automatically generated captions may contain errors.

Video Figure (Optional):
You can submit an accompanying video figure with up to 5 minutes as a .mp4 file. See Technical Requirements and Guidelines for Videos at CHI for details.

Video Figure Captions (Required if the video figure contains spoken dialog): 
Subtitle file in .srt format. A manually created caption file is strongly recommended as automatically generated captions may contain errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End: General Information %%%%%%%%%%%%%%%%%%%%%%%%



==> Charts/DifferentApproachVisualization.tex <==

\begin{figure}[t]  

\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar, axis on top,
        height=7cm, width=8.2cm,
        bar width=0.5cm,
        ymajorgrids, tick align=inside,
        major grid style={draw=white},
        enlarge y limits={value=.1,upper},
        ymin=0, ymax=100,
        axis x line*=bottom,
        axis y line*=right,
        y axis line style={opacity=0},
        tickwidth=0pt,
        enlarge x limits=true,
        enlarge x limits={abs=2cm}, 
        legend style={
            at={(0.5,-0.1)},
            anchor=north,
            legend columns=-1,
            /tikz/every even column/.append style={column sep=0.5cm}
        },
        ylabel={F1-measure (\%)},
        symbolic x coords={
           Classification},
       xtick=data,
       nodes near coords={
        \pgfmathprintnumber[precision=0]{\pgfplotspointmeta}
       }
    ]
    \addplot [draw=none, fill=blue!30] coordinates {
      (Classification,92)
      };
   \addplot [draw=none,fill=red!30] coordinates {
      (Classification,64)
      };
   \addplot [draw=none, fill=green!30] coordinates {
      (Classification,2.3)
       };

    \legend{Our approach,Pattern-based, Random classifier}
  \end{axis}
  \end{tikzpicture}
  \caption{Visualization of the F1-measure for Different Approaches. \eman{do you need this figure? shall we just keep Table 6 since it has the same information?}} \Murtaza{If it does not hurt anything, let's keep it because it highlights F-1 measures. The table presents multiple stats}
\label{Chart:Visualization of the F1-measure for Different Approaches}
  \end{figure}
  



==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> RebuttalResponse.tex <==
Paper Revisions:

#### Clarify the cross-validation hold out testing set in sec 3.5
Section 3.5, Page 8, Line 822-828

#### Add details about the ML models in sec 3.4
Section 3.4, Page 6, Line 616-654

#### Add examples for false positives and false negatives in sec 4
Section 4, Page 8, Line 907-927 + Table 5

#### Provide further analysis on the misspelled words in sec 4
Section 4, Page 8, Line 901-919 + Table 5

#### Provide more details on the features (e.g., keywords, context, semantics) used by the ML model in sec 4
Section 3.3, Page 5, Line 578-589
Section 4, page 8, Line 887-900 + Tables 3 & 4

#### Add a link to the public service and the dataset, in sec 1.
Section 1, Page 1, Line 218-220

#### Add details about the dataset and how it is realistic (information about the apps and reviews), in sec 3.1.
Section 3.1, Pages 4 & 5, Line 400-439 + Table 1 & Figure 2

#### Strengthen the discussion on the findings between ML and keyword-based approaches and adding examples of misspelled words to show how keyword-based fails while ML succeeds, in sec 4.2.
Section 4, Pages 11 - 13, Line 1240-1284 + Figure 5

####Elaborate on the paper’s impact by explaining how future research can build on this paper in sec 5.
Section 5, Pages 12 & 13, Line 1372-1440 + Line 1520-1551



******************************************************************
This paper was discussed extensively at the PC meeting. In particular, we discussed the trade-off between novelty (lower for this paper than most papers) and potential benefit to end users (higher for this paper than many papers).

We decided that this paper can be conditionally accepted, assuming that the authors are able to meet the following requests for revision:

(1) The changes promised in the rebuttal should be made
(2) The usefulness of the method in practice was the primary reason for acceptance, but the case for usefulness will need to be improved in the paper. First, the paper should include more discussion about how developers could use the tool in practice (and perhaps even how this may compare to alternative approaches like manually reading the reviews or keywords alone). Second, the paper should add a discussion of the use case of people with disabilities filtering reviews when searching for apps to use. Users with disabilities may benefit from reading accessibility reviews before downloading and trying out an application. This use case convinced many PC members of the immediate utility of the tool.
Section 5, Pages 12 & 13, Line 1372-1440 + Line 1520-1551

This is optional: If at all possible, please open source the code to make the tool even more immediately useful.
Section 1, Page 1, Line 218-220

Finally, thank you to the authors for their thoughtful rebuttal. It helped the PC committee and reviewers to come to a positive decision on the work and provide confidence that the necessary revisions could be made in the time available.

==> Tables/AllKeywords.tex <==
\begin{table*}[tbp]
%	\fontsize{}{}\selectfont
	%\tabcolsep=0.15cm
\begin{center}
\caption{Eler et al. List of all accessibility keywords.}
\label{Table:AllKeywords}

\begin{adjustbox}{width=0.7\textwidth,center}
%\begin{adjustbox}{width=\textheight,totalheight=\textwidth,keepaspectratio}
\begin{tabular}{llll}

\toprule
\textbf{Keywords} \\
         \midrule 
accessibility           & control key               & light mode                & spacing \\
accessible              & customization             & light theme               & speech synthesizer\\
actionable              & dark mode                 & link description          & stop button\\
adaptability            & dark theme                & logical order             & strain\\
adaptable               & decorative background     & logical sequence          & subtitle\\
adjust color            & decorative content        & magnify                   & suplementary information\\
adjust colour           & decorative element        & metadata                  & svg image\\
adjust font             & decorative image          & migraine                  & switch device\\
adjust size             & default input format      & minimum space             & talkback\\
adjustability           & default language          & missing image             & target area\\
adjustable              & difficult to read         & missing label             & text alternative\\
alert dialog            & difficult to see          & missing layout            & text equivalent\\
alternative format      & disabled person           & mute                      & text reflow\\
alternative text        & disabled user             & narrative audio           & text resize\\
animated content        & disorientating            & nausea                    & text resizing\\
aria label              & disorientation            & navigable                 & text size\\
assistance              & distinguishable           & navigational aids         & text-to-speech\\
assistive               & dizziness                 & night mode                & timeout\\
audible content         & duplicate link            & no label                  & timing out\\
audio conflict          & epilepsy                  & non actionable            & tiny font\\
audio cue               & explicit labels           & non executable            & too bright\\
audio description       & eyestrain                 & non text                  & tooltip\\
auto-play               & fatigue                   & non visual                & touch size\\
autoplay                & flicker                   & non-actionable            & touch target\\
background color        & focus order               & non-executable            & transcript\\
background colour       & focusable                 & non-text                  & understandable\\
background image        & font size                 & non-visual                & unexpect open\\
black mode              & font sizing               & older device              & unexpected audio\\
black theme             & grouped                   & operable                  & unexpectedly opening\\
blind                   & haptic                    & overlap                   & unfamiliar\\
button order            & hard to see               & page refresh              & unique description\\
can't read              & have focus                & page title                & unique label\\
can't see               & headache                  & pause button              & unsupported style\\
cannot read             & header                    & perceivable               & verbose\\
cannot see              & heading                   & personalization           & verbosity\\
captcha                 & hearing loss              & photosensitive            & vertigo\\
change focus            & hidden text               & play automatic            & vibration alert\\
change font             & images of text            & plays automatic           & vibration feedback\\
change language         & impaired                  & properly grouped          & visible focus\\
choose language         & impairment                & readable                  & visible label\\
clear error message     & impossible to read        & repeated link             & vision impairment\\
clear label             & impossible to see         & scaling                   & visual cue\\
colour coding           & inactive space            & screen glare              & visual formatting\\
complex control         & input method              & screen reader             & voice command\\
component order         & input sign                & screen title              & volume\\
consistency             & input type                & screenreader              & wcag\\
consistent label        & keyboard language         & seizures                  & white mode\\
container               & keyboard trap             & select language           & white theme\\
content description     & label absent              & self voicing              & widget order\\
content order           & label place               & sign language             & zoom\\
content resizing        & landmark                  & small button\\
contentDescription      & large font                & small control\\
contrast                & larger font               & small font\\
control focus           & leave focus               & small widget\\




   

        
        \bottomrule
\end{tabular} 
\end{adjustbox}
\end{center}
%\vspace{-2mm}
\end{table*}
%\afterpage{\FloatBarrier}







==> Tables/BinaryClassifiers.tex <==



\begin{table}[h]
\begin{center}
\caption{Performance of %\yasmine{our tested?eman{done}} 
our tested binary classifiers.} %\eman{highlight or bold the classifier with best performance}\Murtaza{Text Bolded}}
\label{Table:binary classifiers}
%\begin{adjustbox}{width=1.1\columnwidth,center}
\begin{tabular}{lcccc}\hline
\toprule
%\multicolumn{2}{l}{\textbf{\textit{Model Building Phase}}}\\
\bfseries Classifier & \bfseries Accuracy & \bfseries Precision & \bfseries Recall  & \bfseries F1-measure   \\



\midrule
Logistic Regression                             & 0.881    & 0.920     & 0.834     & 0.875 \\
Decision Forest                                 & 0.880    & 0.914     & 0.838     & 0.874 \\
\textbf{Boosted Decision Tree}                           & \textbf{0.906}    & \textbf{0.898}     & \textbf{0.916}     & \textbf{0.907} \\
Neural Network                                  & 0.854    & 0.825     & 0.901     & 0.860 \\
Support Vector Machine                          & 0.869    & 0.892     & 0.840     & 0.865 \\
Averaged Perceptron                             & 0.886    & 0.903     & 0.864     & 0.883 \\
Bayes Point Machine                             & 0.889    & 0.906     & 0.869     & 0.887 \\
Decision Jungle                                 & 0.870    & 0.914     & 0.818     & 0.863 \\
Locally Deep SVM                                & 0.873    & 0.882     & 0.860     & 0.871 \\

\bottomrule



  


\end{tabular}
%\end{adjustbox}
\end{center}

\end{table}









==> Tables/CodingGuide.tex <==
\begin{table*}[h]
\begin{center}
\caption{Patterns of accessibility and non-accessibility reviews.} %\eman{Is there any interesting observation we can draw from the manual analysis? Any overlapping keywords? Would it be possible to show example for each in the same table?}}\Murtaza{There could have been some interesting patterns but I did not have it in mind while manually looking for accessibility reviews. Again, keyword extraction is not part of this work. It might be possible, but do we have to?}
\label{Table:Coding Guide}
\begin{adjustbox}{width=1.4\columnwidth,center}
\begin{tabular}{ll}\hline
\toprule
%\multicolumn{2}{l}{\textbf{\textit{Model Building Phase}}}\\
\bfseries Accessibility Reivew & \bfseries Non-accessibility Review  \\


\midrule
If the context is about accessibility                               & Only mention of usability feature   \\
Mention of accessibility feature + praise or complaint              & Only mention of accessibility app name   \\
Mention of accessibility feature + accessibility hint               & Mention of accessibility app name + praise or complaint \\
Mention of usability feature + accessibility hint                   & Mention of customer support + insult or complaint  \\
Mention of assistive technology + praise or complaint               & Mention of usability feature + praise or insult  \\
Mention of assistive technology + accessibility hint                & Only mention of accessibility features  \\
Mention of accessibility app + accessibility hint                   & Only mention of assistive technology  \\
Accessibility hint + praise or complaint                            & Accessibility hint only  \\

\bottomrule



\end{tabular}
\end{adjustbox}
\end{center}

\end{table*}




==> Tables/DatasetTable.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
% \resizebox{\columnwidth}{!}{%
\caption{Statistics of the datasets.}
\label{Table:DataCollection}
\begin{adjustbox}{width=1.0\columnwidth,center}

\begin{tabular} {|c|c|c|}\hline
{\cellcolor{lightgray}\textbf{Reviews Type}} & {\cellcolor{lightgray}\textbf{Eler et al. Dataset}} & {\cellcolor{lightgray}\textbf{Our Dataset}} \\ 
 \hline

{\cellcolor{lightgray}\textbf{Non-Accessibility}}    & 211,390   & 2,663  \\ \hline
{\cellcolor{lightgray}\textbf{Accessibility}}        & 2,663     & 2,663   \\ \hline
{\cellcolor{lightgray}\textbf{Total}}                & 214,053   & \textbf{5,326}   \\ \hline

\end{tabular}
% }
\end{adjustbox}
\end{table}

==> Tables/TrainingSize.tex <==
\begin{table}[h]
\begin{center}
\caption{Training dataset.}%\eman{why do we have this table twice? Table 3 \& 7}\Murtaza{Removed one}
\label{Table:TrainingSize}
%\begin{adjustbox}{width=1\columnwidth,center}
\begin{adjustbox}{width=1\columnwidth,center}
\begin{tabular}{cccc}\hline
\toprule
 
%\bfseries Accessibility Reviews & \bfseries \multicolumn{2}{l}{\textbf{Non-accessibility Reviews}}  &  \bfseries Total\\
\bfseries Accessibility Reviews & \bfseries Non-accessibility Reviews  &  \bfseries Total\\

\midrule
%        & with accessibility keywords     & without accessibility keywords      &  \\
%\textbf{2663}    & \textbf{1331}              & \textbf{1332}                  & \textbf{5326} \\
2663            & 2663                  &  5326 \\
\bottomrule



\hline
\end{tabular}
\end{adjustbox}
\end{center}

\end{table}







==> Tables/dataset.tex <==
\begin{table*}[h]
\begin{center}
\caption{\eman{Dataset overview.}}
\label{Table:dataset}
%\begin{adjustbox}{width=1.0\textwidth,center}

\begin{tabular}{lccccccc}\hline
\toprule
\multicolumn{5}{l}{\textbf{Number of reviews and accessibility reviews grouped by category.}} \\
\midrule
\multicolumn{5}{c}{\textit{Information about the apps and reviews (extracted from Eler et al. \cite{eler_android_2019})}} \\
\bfseries Category & \bfseries Apps & \bfseries Reviews & \bfseries Acc. Rev.  & \bfseries Man. Val.  \\

Connectivity & 40 & 5789            & 123   & 58     \\
Development & 25 & 8017             & 130   & 57    \\
Games & 70 & 30109                  & 588   & 314   \\
Graphics & 6 & 981                  & 14    & 3    \\
Internet & 135 & 34662              & 635   & 380  \\
Money & 24 & 5573                   & 92    & 45    \\
Multimedia & 100 & 48020            & 1366  & 555    \\
Navigation & 48 & 4193              & 138   & 51    \\
Phone and SMS & 8 & 9070            & 256   & 176    \\
Reading & 39 & 20308                & 755   & 478  \\
Science and Education & 54 & 12466  & 164   & 114   \\
Security & 39 & 7053                & 192   & 24     \\
Sports and Health & 29 & 7066       & 143   & 80    \\
Time & 42 & 7516                    & 163   & 88    \\
Writing & 42 & 13230                & 347   & 240   \\ 
\textbf{Total} & \textbf{701} & \textbf{214053} & \textbf{5076} & \textbf{2663}  \\
\midrule
\multicolumn{5}{c}{\textit{Statistics of the datasets}} \\
\bfseries Review Type & \bfseries Eler et al. &  \bfseries Our dataset\\ \hline
Non-Accessibility & 211,390 & 2,663 \\
Accessibility & 2,663 & 2,663 \\
\textbf{Total} & \textbf{214,053} & \textbf{5,326} \\
\bottomrule
\hline
\end{tabular}
%\end{adjustbox}
\end{center}

\end{table*}



















\begin{comment}

\begin{table*}[h]
\begin{center}
\caption{\eman{Number of reviews and accessibility reviews grouped by category (extracted from Eler et al. \cite{eler_android_2019}).}} %\eman{we need to remove this table since it is taken from previous work [1]}\Murtaza{Removed}
\label{Table:dataset}
\begin{adjustbox}{width=1.0\textwidth,center}

\begin{tabular}{lccccccc}\hline
\toprule
\bfseries Category & \bfseries Apps & \bfseries Reviews & \bfseries Acc. Rev.  & \bfseries Man. Val.  & \bfseries Request & \bfseries Compliment & \bfseries Apps reviewed\\


\midrule
Connectivity & 40 & 5789            & 123   & 58    & 45    & 13    & 12 \\
Development & 25 & 8017             & 130   & 57    & 53    & 4     & 10 \\
Games & 70 & 30109                  & 588   & 314   & 294   & 20    & 31 \\
Graphics & 6 & 981                  & 14    & 3     & 3     & 0     & 2  \\
Internet & 135 & 34662              & 635   & 380   & 296   & 84    & 51 \\
Money & 24 & 5573                   & 92    & 45    & 42    & 3     & 7  \\
Multimedia & 100 & 48020            & 1366  & 555   & 458   & 97    & 47 \\
Navigation & 48 & 4193              & 138   & 51    & 45    & 6     & 11 \\
Phone and SMS & 8 & 9070            & 256   & 176   & 87    & 89    & 5  \\
Reading & 39 & 20308                & 755   & 478   & 296   & 182   & 25 \\
Science and Education & 54 & 12466  & 164   & 114   & 94    & 20    & 20 \\
Security & 39 & 7053                & 192   & 24    & 19    & 5     & 10 \\
Sports and Health & 29 & 7066       & 143   & 80    & 33    & 47    & 6  \\
Time & 42 & 7516                    & 163   & 88    & 77    & 11    & 13 \\
Writing & 42 & 13230                & 347   & 240   & 176   & 64    & 26 \\


\bottomrule
Total & 701 & 214053 & 5076 & 2663 & 2018 & 645 & 276 \\


\hline
\end{tabular}
\end{adjustbox}
\end{center}

\end{table*}
\end{comment}










==> Tables/keyword-basedMeasures.tex <==


%\textit{tp}     & 243   \\
%\textit{tn}     & 509   \\
%\textit{fp}     & 248 \\
%\textit{fn}     & 0 \\







\begin{table}
\begin{center}

\label{Table:Keyword-basedMeasures}
\caption{\yasmine{This table needs a caption and descriptive headers}}
\begin{adjustbox}{width=0.2\columnwidth,center}
\begin{tabular}{cc}




\midrule
\textit{tp}     & 243   \\
\textit{tn}     & 509   \\
\textit{fp}     & 248 \\
\textit{fn}     & 0 \\


\bottomrule

\end{tabular}
\end{adjustbox}
\end{center}

\end{table}

